Towards Code Generation from BDD Test Case Specifications: A Vision

Automatic code generation has recently attracted large attention and is becoming more significant to the software development process. Solutions based on Machine Learning and Artificial Intelligence are being used to increase human and software efficiency in potent and innovative ways. In this paper, we aim to leverage these developments and introduce a novel approach to generating frontend component code for the popular Angular framework. We propose to do this using behavior-driven development test specifications as input to a transformer-based machine learning model. Our approach aims to drastically reduce the development time needed for web applications while potentially increasing software quality and introducing new research ideas toward automatic code generation.

==> sota.tex <==
In the following Section, an overview of the state-of-the-art work in the field of AI4CA is given and current areas of research are highlighted. We will begin with Data Collection followed by discussing different approaches for Auto-Completion and Code Generation, then AI Approaches and finally give an insight into the domain of testing in combination with AI since we deem it crucial for understanding the approach of this paper.

\subsection{Data Collection}

A crucial aspect of ML research is how data used for training, testing, and validation is collected and represented. In the context of code processing there currently exist several approaches for data retrieval and transformation into representations that can then be processed by ML algorithms. \\
When choosing input data for AI tasks in the domain of code analysis, source code is very likely the most obvious choice. Because of the abundance of open-source projects on websites like GitHub \cite{github} or StackOverflow \cite{stackoveflow}, this data is free for anyone to use as input for their ML project. However, directly using text artifacts as an input to further ML steps introduces challenges. This is different from natural language since code follows strict syntactic and semantic rules which allow even slight variations of the input to either render code invalid or have it convey vastly different meanings.\\
One possibility is to decompose the source code into either a string of tokens (token sequence) or an Abstract Syntax Tree (AST). These representations can then be processed by various ML models that require sequential input, such as Recurrent Neural Networks (RNN) \cite{rnn} or Transformer networks \cite{AttentionIsAllYouNeed} to facilitate applications such as next token prediction \cite{kim2021code}. Some applications require further processing to eliminate undesirable data, for example, discarding all Java classes with missing documentation \cite{iyer2018mapping}. \\
Most current approaches rely on such local representations of the code like ASTs or tokens \cite{allamanis17}. However, if broad usage patterns are to be captured across multiple programs such local representations may not be appropriate. Abdelaziz et al. \cite{abdelaziz20} propose a method to statically extract control and data flow information and aggregate it in a knowledge graph. This way data from multiple programs can be stored loosely coupled in a single knowledge base which allows queries to be performed to extract information invariant to local representations. \\
While some work \cite{6693113, iyer-etal-2016-summarizing} just rates the quality of an answer based on its rating, more recent work \cite{DBLP:journals/corr/abs-1805-08949} uses generalized classification frameworks with hand-crafted features and test datasets as well as state-of-the-art RNN approaches. The extracted information can be further processed by integrating data extracted from code and documentation to build a unified knowledge graph that can serve as a general-purpose data set for various applications.~\cite{abdelaziz20} \\
Another useful source of data is the current programming environment. Information like class members and data types can take an essential role during code generation because it can be used along with natural language to predict the next piece of code. For example, the model can call or use already existing methods in a class instead of writing new code that is doing the same task as an existing method.~\cite{iyer2018mapping}

\subsection{Auto-Completion and Code Generation}
Most of the current research and techniques described in this paper are related to how AI can be used either for better auto-completion \cite{UMLTM, pythia, kim2021code, svyatkovskiy2020intellicode} or the generation of code segments \cite{https://doi.org/10.48550/arxiv.2107.03374, iyer2018mapping}. \\
The latter generates code from scratch using doc-strings, user annotations, and signatures. Chen et al.~\cite{https://doi.org/10.48550/arxiv.2107.03374} propose a method to generate code from hand-written doc-strings or function signatures using a generative pre-trained transformer (GPT)~\cite{gpt} model by the name of Codex. To ensure the correctness of the produced function, it is analysed using several hand-written gold standard test cases. Furthermore, Codex can generate doc-strings using pre-defined functions. In contrast to generated code sequences, the generated doc-strings have to be evaluated manually. Unfortunately, despite using a large amount of training data, Codex struggles with long or high-level descriptions or specifications of functions. Additionally, code created by Codex can contain unintended side effects and introduce security risks.\\
Another approach for generating code snippets is described in the work by Iyer et al. \cite{iyer2018mapping}. Similar to Codex, it uses information from doc-strings (function description, return type) and function signatures to generate function bodies. Furthermore, class member variables, member functions, and natural language documentation for methods are utilized. To perform this, the generation process is split into two steps: First, the class components are encoded using high-dimensional vectors and n-Layer bidirectional Long Short-Term Memory (Bi-LSTM) \cite{lstm}. Second, ASTs are derived to create a set of production rules which define how a sequence of source code is generated. A supervised copy mechanism is used to process the production rules to recognize the members that can be copied from the class environment. \\
To ease the programming process, Integrated Development Environments (IDEs) introduce Code Completion. Instead of generating whole function bodies or big code snippets, code completion just predicts the next code element or token in a source code sequence \cite{UMLTM} and creates a list of possible predictions. Typically, code completion is performed through popups that display a list of the most likely methods, functions, variables, or parameters while typing. Most of the code completion approaches presented in this paper utilize some form of Abstract Syntax Trees (ASTs) to collect structural and hierarchical information.\\
The Unified Multi-Task learning-based neural Language Model for code completion (UMTLM) \cite{UMLTM} and Pythia \cite{pythia} encode AST nodes, as well as tokens of the source to create embeddings that represent particular code elements. Vector representations of tokens or AST nodes are used since they are effective in natural language processing (NLP). These embeddings are then processed by several ML techniques to predict code. Furthermore, UMTLM involves Multi-task learning to either jointly predict type and value or estimate the type first and use it to predict the value. Additionally, Pythia can handle aliasing used in Python code. \\
Recent work by Kim et. al. \cite{kim2021code} also focuses on the task of code completion. In this approach, ASTs are processed by several transformer models: \textit{SeqTrans}, \textit{PathTrans} and \textit{TravTrans}. ASTs are decomposed into partial ASTs by PathTrans and TravTrans. PathTrans feeds the root path of each AST to the transformer whereas TravTrans transforms the partial ASTs using preorder traversal. \\
All the described Code Completion approaches try to prioritize the most likely next code element and rank them first based on the used techniques and workflow, in contrast to na\"ive approaches that, for example, just create alphabetically sorted predictions. Moreover, some of the approaches described above can be used to create and collect training data for the approaches mentioned in the current Section. A mix of features discovered by ML models combined with handcrafted, language-independent features can be a suitable solution for training and testing Auto-Completion and Code Generation systems \cite{abdelaziz21, DBLP:journals/corr/abs-1805-08949}.

\subsection{AI Approaches}
Usually, the task of language generation consists of three stages: sentence pre-processing, encoding, and decoding \cite{iyer2018mapping,kim2021code}. The pre-processing stage focuses on tokenizing a sentence correctly and/or generating an AST, whereas the encoding stage translates sentence sequences into word embedding. The decoding stage translates word embeddings back into sentence sequences. Most AI approaches that aim to generate code are focused on these stages. \\
As mentioned in the previous sections, code is often represented as an AST but most models like Transformers and RNNs used in NLP are developed for sequential data. To combat this mismatch several techniques were developed that enable ASTs to be used in conjunction with these kinds of models. An empirical study by Chirkova et al. \cite{ESoTfSC} compares different mechanisms for feeding ASTs to Transformers and describes that augmenting self-attention \cite{AttentionIsAllYouNeed} with relative position representations (Sequential Relative Attention \cite{sra}) is the best mechanism to use them and syntactic information. Depending on the task, combination with other mechanisms, e.g. Gated Graph Sequence Neural Networks (GGNN) Sandwich \cite{ggnn-sandwich} or tree relative attention \cite{tra} to tweak the performance is possible. \\
Yin et al. \cite{DBLP:journals/corr/abs-1805-08949} propose a classifier that determines how well a pair of code and a question fit together. In this work, features are retrieved from RNNs and then combined with hand-crafted ones that obey language-independent rules. Some Transformers integrate the encoder stage and decoder stage, e.g. GPT, and BERT models. Chen et al. \cite{https://doi.org/10.48550/arxiv.2107.03374} also use GPT to do sentence prediction while Svyatkovskiy et al. \cite{svyatkovskiy2020intellicode} establish GPT-C, a modification of GPT-2 trained from scratch on source code data.


\subsection{Testing and AI}
AI is widely used in the domain of software testing. It comes in varieties from a suggestion of assert statements \cite{DBLP:journals/corr/abs-2009-05634} to automated test case generation (TCG) \cite{10.1145/1353673.1353674} or automatic building of documentation based on test cases \cite{https://doi.org/10.48550/arxiv.2005.08750}. As depicted in the introduction, the reduction of necessary manual effort is the most reported benefit of automated TCG compared to writing them by hand \cite{Trudova2020ArtificialII}. In general, state-of-the-art TCG uses evolutionary algorithms since they mimic the iterative process of a developer the best \cite{9793774}. \\
While most approaches of TCG are generating test cases only from code \cite{DBLP:journals/corr/abs-2009-05634, 10.1145/1353673.1353674, https://doi.org/10.48550/arxiv.2005.08750}, there are a few other approaches that use e.g. natural language in combination with code as a baseline for TCG. As mentioned in earlier chapters, transformers represent the state of the art in many areas of AI4CA. Thus, transformers are also frequently used in TCG. \\
In the case of \cite{DBLP:journals/corr/abs-2009-05634}, a BART transformer \cite{DBLP:journals/corr/abs-1910-13461} is used, which is pre-trained on an English text corpus. By further pretraining with large amounts of code, significant performance boosts are achieved compared to conventional methods for the generation of assert statements. TCG tasks can be treated as a translation task to translate, e.g. from a partially written unit test and a method to an assert statement as a suggestion. \\
A similar approach is taken when using AI planners to generate unit tests for Java classes with varying sizes and semantics \cite{10.1145/1353673.1353674}. Here the problem again is treated as a translation task from a Java class, its method specifications as Javadoc and a desired unit test goal as input, and a Java Unit Test Case as a target. In other work, no AI is used to detect and replace outdated documentation based on the test suite for the software \cite{https://doi.org/10.48550/arxiv.2005.08750}. \\
In older work~\cite{Soeken2012}, researchers generate code stubs from behaviour-driven development (BDD) tests by using NLP techniques that do not incorporate a ML model.
They extract relevant information need for the stub generation by using a Phase Structure Tree (PST) in combination with the text corpus of WordNet \cite{wordnet}.
